Multi-blank Transducers for Speech Recognition

This paper proposes a modification to RNN-Transducer (RNN-T) models for automatic speech recognition (ASR). In standard RNN-T, the emission of a blank symbol consumes exactly one input frame; in our proposed method, we introduce additional blank symbols, which consume two or more input frames when emitted. We refer to the added symbols as big blanks, and the method multi-blank RNN-T. For training multi-blank RNN-Ts, we propose a novel logit under-normalization method in order to prioritize emissions of big blanks. With experiments on multiple languages and datasets, we show that multi-blank RNN-T methods could bring relative speedups of over +90%/+139% to model inference for English Librispeech and German Multilingual Librispeech datasets, respectively. The multi-blank RNN-T method also improves ASR accuracy consistently. We will release our implementation of the method in the NeMo (https://github.com/NVIDIA/NeMo) toolkit.

==> graph_plot.tex <==
\begin{figure}[t]
\hspace{-3pt}
\begin{tikzpicture}
\pgfplotsset{%
    x tick label style={/pgf/number format/1000 sep=\,},
    log base 10 number format code/.code={%
        $\pgfmathparse{10^(#1)}\pgfmathprintnumber{\pgfmathresult}$%
    }%
}  
\begin{axis}[
    xmode=log,
    log ticks with fixed point,
    xlabel={Vocabulary size [number of wordpieces]},
    ylabel={Graph size [GiB]},
    height=6.5cm,
    xmin=128, xmax=2048,
    ymin=4, ymax=24,
    xtick={128,256,512,1024,2048},
    xticklabels={128,256,512,1024,2048}, % latex incorrectly displays logarithmic ticks
    ytick={5,8,11,14,17,20,23},
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
	enlargelimits=0.025,
]

\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (128,16.686580021)(256,16.210114081)(512,12.958632869)(1024,11.360642777)(2048,9.374569253)};
    \addlegendentry{TLG.fst}

\addplot[
    color=brown,
    mark=halfcircle,
    ]
    coordinates {
    (128,21.951218701)(256,18.518031621)(512,15.936703145)(1024,13.494135421)(2048,10.690085437)};
    \addlegendentry{T\textsubscript{\scalebox{1.2}{eesen}}LG.fst}

\addplot[
    color=green,
    mark=triangle,
    ]
    coordinates {
    (128,13.454113621)(256,11.590339129)(512,10.177699053)(1024,8.813753657)(2048,7.180788233)};
    \addlegendentry{T\textsubscript{\scalebox{1.2}{compact}}LG.fst}

\addplot[
    color=blue,
    mark=diamond,
    ]
    coordinates {
    (128,8.253983465)(256,7.316065853)(512,6.594173965)(1024,5.867700781)(2048,4.931680801)};
    \addlegendentry{T\textsubscript{\scalebox{1.2}{minimal}}LG.fst}

\addplot[
    color=black,
    mark=star,
    dashed]
    coordinates {
    (128,6.414693433)(256,5.775879145)(512,5.303925905)(1024,4.915517181)(2048,4.568019881)};
    \addlegendentry{LG.fst}

\end{axis}
\end{tikzpicture}
%\vspace{-25pt} % adjust this
\vspace{-20pt} % adjust this
\caption{Decoding graph sizes with the considered topologies.}
\label{fig:graph-plot}
\vspace{-15pt} % adjust this
\end{figure}


% data
% correct: arcs[769667056,763880501,615276649,546992982,458390283] states[218595353,199401300,155710321,130437750,102016233] size[16686580021,16210114081,12958632869,11360642777,9374569253]
% eesen: arcs[850391361,725126731,630790485,540320351,433968267] states[417247843,345800193,292202766,242450487,187329655] size[21951218701,18518031621,15936703145,13494135421,10690085437]
% no selfloops: arcs[652025108,664179852,529217612,473743121,399820617] states[218595353,199401300,155710321,130437750,102016233] size[14804308853,14614903697,11581688277,10188645001,8437454597]
% compact: arcs[568826531,497023424,442389958,388478692,321522093] states[217644453,181898214,154972983,129904726,101821734] size[13454113621,11590339129,10177699053,8813753657,7180788233]
% minimal: arcs[368821525,332628298,304562070,275168966,235017961] states[117641950,99700651,86059039,73249863,58569668] size[8253983465,7316065853,6594173965,5867700781,4931680801]
% LG: arcs[252984303,235332235,222307595,211601871,202026046] states[118347226,100528166,87350216,76494359,66780154] size[6414693433,5775879145,5303925905,4915517181,4568019881]

==> topo_pics_src.tex <==
\def\greps{\detokenize{〈}\detokenize{ε}\detokenize{〉}}
\def\grblk{\detokenize{〈}b\detokenize{〉}}

\begin{figure*}[ht]
\vspace{-25pt} % adjust this
\hspace{-20pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{default2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<a) T.fst> labelloc=b center=1 nodesep=0.25 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
    0 -> 0 [label="\grblk:\greps"]
	1 [label=1 shape=doublecircle]
	0 -> 1 [label="A:A"]
	2 [label=2 shape=doublecircle]
	0 -> 2 [label="B:B"]
	1 -> 0 [label="\grblk:\greps"]
	1 -> 1 [label="A:\greps" style="dashed"]
	1 -> 2 [label="B:B"]
	2 -> 0 [label="\grblk:\greps"]
	2 -> 1 [label="A:A"]
	2 -> 2 [label="B:\greps" style="dashed"]
}
\label{fig:topologies_a}
\endminipage\hfill
\hspace{+17pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{eesen2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<b) T<SUB>eesen</SUB>.fst> labelloc=b center=1 nodesep=0.25 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
	1 [label=1 shape=circle]
	0 -> 1 [label="\greps:\greps"]
	1 -> 1 [label="\grblk:\greps"]
	3 [label=3 shape=circle]
	1 -> 3 [label="A:A"]
	4 [label=4 shape=circle]
	1 -> 4 [label="B:B"]
	2 [label=2 shape=circle]
	2 -> 0 [label="\greps:\greps"]
	2 -> 2 [label="\grblk:\greps"]
	3 -> 2 [label="\greps:\greps"]
	3 -> 3 [label="A:\greps" style="dashed"]
	4 -> 2 [label="\greps:\greps"]
	4 -> 4 [label="B:\greps" style="dashed"]
}
\label{fig:topologies_b}
\endminipage\hfill
\hspace{+65pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{compact2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<c) T<SUB>compact</SUB>.fst> labelloc=b center=1 nodesep=0.25 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
	0 -> 0 [label="\grblk:\greps"]
	1 [label=1 shape=circle]
	0 -> 1 [label="A:A"]
	2 [label=2 shape=circle]
	0 -> 2 [label="B:B"]
	1 -> 0 [label="\greps:\greps"]
	1 -> 1 [label="A:\greps" style="dashed"]
	2 -> 0 [label="\greps:\greps"]
	2 -> 2 [label="B:\greps" style="dashed"]
}
\label{fig:topologies_c}
\endminipage\hfill
\hspace{-56pt} % adjust this
\minipage[t]{0.2\textwidth}
  \digraph[scale=0.5]{minimal2}{
    graph [fontname = "times" fontsize=18];
    node [fontname = "times" fontsize=18];
    edge [fontname = "times" fontsize=18];
	graph [label=<d) T<SUB>minimal</SUB>.fst> labelloc=b center=1 nodesep=0.4 orientation=Portrait rankdir=LR ranksep=0.35 size="8.5,11"]
	0 [label=0 shape=doublecircle style=bold]
	0 -> 0 [label="\grblk:\greps" headport=e tailport=w]
	0 -> 0 [label="A:A" headport=e tailport=w]
	0 -> 0 [label="B:B" headport=e tailport=w]
}
\label{fig:topologies_d}
\endminipage
\hspace{-24pt} % adjust this
\vspace{-40pt} % adjust this
\caption{Example CTC topologies for a three-unit vocabulary: $\langle blank \rangle$, $A$, and $B$. Variants: a) correct-CTC, b) Eesen-CTC, c) compact-CTC, d) minimal-CTC. $\langle b \rangle$ states for $\langle blank \rangle$. Language unit-to-$\langle \epsilon \rangle$ selfloops are indicated by dashed arrows.}
\label{fig:topologies}
\vspace{-15pt} % adjust this
\end{figure*}

